Opinion Control under Adversarial Network Perturbation: A Stackelberg Game Approach

The emerging social network platforms enable users to share their own opinions, as well as to exchange opinions with others. However, adversarial network perturbation, where malicious users intentionally spread their extreme opinions, rumors, and misinformation to others, is ubiquitous in social networks. Such adversarial network perturbation greatly influences the opinion formation of the public and threatens our societies. Thus, it is critical to study and control the influence of adversarial network perturbation. Although tremendous efforts have been made in both academia and industry to guide and control the public opinion dynamics, most of these works assume that the network is static, and ignore such adversarial network perturbation. In this work, based on the well-accepted Friedkin-Johnsen opinion dynamics model, we model the adversarial network perturbation and analyze its impact on the networks' opinion. Then, from the adversary's perspective, we analyze its optimal network perturbation, which maximally changes the network's opinion. Next, from the network defender's perspective, we formulate a Stackelberg game and aim to control the network's opinion even under such adversarial network perturbation. We devise a projected subgradient algorithm to solve the formulated Stackelberg game. Extensive simulations on real social networks validate our analysis of the adversarial network perturbation's influence and the effectiveness of the proposed opinion control algorithm.

==> method.tex <==
\section{methods}
In this section, we solve the robust opinion minimization problem in \refeq{eqn:rocpi}. To solve \refeq{eqn:rocpi}, we first need to solve the inner maximization problem.
This corresponds to asking what are the optimal attacker set $\mathcal{A}$ and their optimal target users $\mathcal{T}_u^*$ for each optimal attacker $u\in \mathcal{A}^*$.
Next, based on the optimal attackers and target users, we solve the outer minimization problem by the defender.

\subsection{Optimal Attackers and Target Users}


%%%%%%%%% previous %%%%%%%%%%
% In this section, we investigate the proposed two robust opinion control problem: ROCPI and ROCII. We theoretically analyze how the worst case is reached in both problems and design effective algorithm to solve them.
% % Since the network perturbation may happens during the opinion dynamics, the original opinion control algorithm in \cite{xu2020opinion} may not work anymore.
% % In this section, we take the network perturbation into consideration, and build a robust opinion minimization algorithm.

% % From the defense's perspective, their goal is to minimize the total opinion at equilibrium $\tilde{f}$.
% % However, the attacker $m$ and the target user set $\mathcal{T}$ remains unknown for the defense.
% % From the game theoretical perspective, the defense may assume that perturbation is conduct by a ``rational adversary'' whose goal is to maximize the total opinion at equilibrium.

% \subsection{The Worst Network Perturbation}
% \label{sec:worst-net-perturb}
% We first analyze the worst case among all potential network perturbations when the size of source user set $\vert \mathcal{S} \vert$ is known.
% That is, we solve the maximization term in \refeq{eqn:rocpi}.
% To achieve this, we need to find out the optimal source user set $\mathcal{S}^*$, each source user $v$'s optimal target users $\mathcal{T}_v^*$, and the optimal influence weight of them $p^*_{uv}$.

% According to \refprop{prop:approx-new-total}, we first have
% \begin{equation}
%   \begin{aligned}
%     \tilde{f} &\approx \mb{1}^T \mb{B} \mb{A} \mb{s} + p\times \mb{1}^T \mb{B} (\mb{I} - \mb{A}) \mb{\Delta}_{W} \mb{B} \mb{A} \mb{s}\\
%     &= f + p\times \mb{1}^T \mb{B} (\mb{I} - \mb{A}) \left(\sum_{v\in \mathcal{S}} \mb{e}_v \left(\sum_{u\in\mathcal{T}_v} \frac{p_{uv}}{p}\cdot \mb{e}_u^T\right)  - \sum_{v\in \mathcal{S}} \mb{e}_v \mb{e}_v^T \mb{W}\right) \mb{B} \mb{A} \mb{s}\\
%     &= f + p\times \mb{c}_1^T \left(\sum_{v\in \mathcal{S}} \mb{e}_v \left(\sum_{u\in\mathcal{T}_v} \frac{p_{vu}}{p}\cdot \mb{e}_u^T \mb{z}^*\right)  - \sum_{v\in \mathcal{S}} \mb{e}_v \mb{e}_v^T \mb{c}_2\right)\\
%     &= f + p\times \sum_{v\in \mathcal{S}} c_1(v) \cdot \left(\sum_{u \in \mathcal{T}_v} \frac{p_{vu}}{p} \cdot z^*(u) - c_2(v)\right)
%   \end{aligned}
%   \label{eqn:new-total-refac}
% \end{equation}
% where $\mb{c}_1^T = \mb{1}^T \mb{B} (\mb{I} - \mb{A})$, $\mb{z}^*=\mb{B}\mb{A}\mb{s}$, and $\mb{c}_2 = \mb{W}\mb{z}^*$.
% We define
% \begin{equation}
%   \delta_v = c_1(v) \cdot \left(\sum_{u \in \mathcal{T}_v} \frac{p_{vu}}{p} \cdot z^*(u) - c_2(v)\right)
% \end{equation}
% as the \textit{individual influence} on the total opinion at equilibrium caused by source user $v$'s perturbation.
% In this way, the change of total opinion is refactored to the sum of each source user $v$'s individual influence $\delta_v$.
% It is worth to mention that, the contribution of each individual influence $\delta_v$ to the change of total opinion is also controlled by the perturbation coefficient $p$.

% We first study the influence of source user $v$, i.e., $\delta_v$.
% Define $m = \arg\max_u z^*(u)$ as the \textit{extreme user} who owns the largest expressed opinion at equilibrium when there is no perturbation.
% Note that $c_1(v) \ge 0$ for any $v \in \mathcal{V}$.
% Therefore, for each individual influence term $\delta_v$, it is maximized when
% \begin{align}
%   \mathcal{T}^*_v &= \{ m \}, \text{ and }
%   p^*_{vu} = \begin{cases}
%     1 & u = m;\\
%     0 & otherwise.
%   \end{cases}
% \end{align}
% Consequently, the optimal individual influence is
% \begin{equation}
%   \delta_v^* = c_1(v) \cdot \left(z^*(m) - c_2(v)\right).
% \end{equation}
% Furthermore, since $c_2(v) = \sum_j W_{vj} \mb{z}^*(j) \le \sum_j W_{vj} \mb{z}^*(m) = \mb{z}^*(m)$, we have $\delta_v^* \ge 0$ for any user $v\in \mathcal{V}$ if $v$ is the source user.

% From the above analysis, we can see that during the network perturbation, if any source user $v$ is only influenced by the extreme user $m$, he/she can always increase the total opinion at equilibrium the most.
% This corresponds to the real scenario that some innocent users happen to read blog posts by those extreme users, then follow their extreme opinions, and further spread their extreme opinions to others.
% The above analysis further validates that the existence of extreme users may pose potential threats to the opinion optimization and further public security.

% Next, we analyze the optimal source user set $\mathcal{S}^*$.
% With the analysis above, we have
% \begin{equation}
%   \tilde{f} = f + p\times \sum_{v\in \mathcal{S}} \delta_v^*.
% \end{equation}
% Therefore, to maximize $\tilde{f}$ with respect to $\mathcal{S}$, we need to choose the top-$k$ users who have the largest optimal individual influence $\delta_v^*$.
% In this sense, we develope a rank $\delta_v^*$ for each user. Since $c_1(v) = (\mb{B}^T\mb{1})_v \cdot (1 - \alpha_v)$ and $c_2(v) = \sum_j W_{vj} z^*_j$, we have the following remarks on the ranking of users.
% First, if a user $v$ has small $\alpha_v$ and is inclined to be influenced by others, he/she tend to have a larger optimal individual influence $\delta_v^*$. Second, if a user $v$'s original neighbors expressed opinion at equilibrium tend to be small, this user tend to have a small $c_2(v)$ value and further a larger optimal individual influence $\delta_v^*$.


% \subsection{Algorithm for ROCPI}
% With the above analysis, the objective function in ROCPI problem \refeq{eqn:rocpi} can be refactored as
% \begin{equation}
%   \begin{aligned}
%     \tilde{f} &= \mb{1}^T \mb{B} \mb{A} \mb{x} + p\times\sum_{l = 1}^k \left(\mb{C} (\bar{z} \mb{1} - \mb{c}_2)\right)_{[l]}\\
%     &= \mb{1}^T \mb{B} \mb{A} \mb{x} + p\times\sum_{l = 1}^k \left( \begin{bmatrix} -\mb{CWBA} & \mb{c}_1 \end{bmatrix} \cdot \begin{bmatrix} \mb{x} \\ \bar{z} \end{bmatrix} \right)_{[l]}
%   \end{aligned}
% \end{equation}
% where $\mb{C} = \Diag{\mb{c_1}}$, $\bar{z} = \max{(\mb{B}\mb{A}\mb{x})}$, and $(\mb{y})_{[l]}$ means the $l$-th largest element in vector $\mb{y}$.
% Consequently, we can transform the ROCPI problem in \refeq{eqn:rocpi} into
% \begin{equation}
%   \begin{aligned}
%     \min_{\mb{x}, \bar{z}} & \quad\mb{1}^T \mb{B} \mb{A} \mb{x} + p\times\sum_{l = 1}^k \left( \begin{bmatrix} -\mb{CWBA} & \mb{c}_1 \end{bmatrix} \cdot \begin{bmatrix} \mb{x} \\ \bar{z} \end{bmatrix} \right)_{[l]}\\
%     s.t.            & \quad 
%     \left\{\begin{array}{lc}
%       \mb{1}^T (\mb{s} - \mb{x}) \le \mu,\\
%       \quad \mb{0} \le \mb{x} \le \mb{s},\\
%       \quad\mb{B} \mb{A} \mb{x} \le \bar{z} \mb{1}.
%     \end{array}\right.
%   \end{aligned}
%   \label{eqn:rocpi-transformed}
% \end{equation}
% Note that the objective in \refeq{eqn:rocpi-transformed} is a linear term plus an $k$-largest components of a linear transformation of decision variables $[\mb{x}, \bar{z}]$. The constraints in \refeq{eqn:rocpi-transformed} are all linear with respect to decision variables. Thus, the ROCPI problem is a convex optimization problem.

% The main challenge to solve \refeq{eqn:rocpi-transformed} is to deal with the $k$-largest components term in objective.
% According to \cite{ogryczak2003minimizing}, the above optimization problem can be transformed into
% \begin{equation}
%   \begin{aligned}
%     \min_{\mb{x}, \bar{z}, \mb{d}, \eta} & \quad\mb{1}^T \mb{B} \mb{A} \mb{x} + p\times (k\eta + \mb{1}^T \mb{d})\\
%     s.t.            & \quad 
%     \left\{\begin{array}{lc}
%       \mb{1}^T (\mb{s} - \mb{x}) \le \mu,\\
%       \quad \mb{0} \le \mb{x} \le \mb{s},\\
%       \quad\mb{B} \mb{A} \mb{x} \le \bar{z} \mb{1},\\
%       \begin{bmatrix} -\mb{CWBA} & \mb{c}_1 \end{bmatrix} \cdot \begin{bmatrix} \mb{x} \\ \bar{z} \end{bmatrix} - \eta \mb{1} \le \mb{d},\\
%       \mb{d} \ge 0
%     \end{array}\right.
%   \end{aligned}
%   \label{eqn:rocpi-linear}
% \end{equation}
% where $\mb{d}$ and $\eta$ are introduced slack variables. The transformed optimization problem in \refeq{eqn:rocpi-linear} is a linear programming, where there are $(2n + 2)$ variables and $(5n + 1)$ inequality constraints. Therefore, we can use interior-point methods \cite{boyd2004convex} to solve it and obtain the optimal controlled internal opinions $\mb{x}^*$.

% \subsection{Algorithm for ROCII}
% To solve ROCII in \refeq{eqn:rocii}, we first define 
% \begin{equation}
%   \tilde{f}_k = \mb{1}^T \mb{B} \mb{A} \mb{x} + p\times\sum_{l = 1}^k \left( \begin{bmatrix} -\mb{CWBA} & \mb{c}_1 \end{bmatrix} \cdot \begin{bmatrix} \mb{x} \\ \bar{z} \end{bmatrix} \right)_{[l]}
% \end{equation}
% as the \textit{worst perturbed total opinion} if the number of source user is $k$.
% Then, the objective in \refeq{eqn:rocii} becomes
% \begin{align}
%   &\mathbb{E}_{k}\left\{ \max_{\substack{\mathcal{S}, \mathcal{T}_v, p_{uv}\\v \in \mathcal{S}, u \in \mathcal{T}_v}} \tilde{f}\right\} = \sum_{\hat{k} = 0}^{n} \lambda(k) \cdot \tilde{f}_{\hat{k}}\nonumber\\
%   &= \mb{1}^T \mb{B} \mb{A} \mb{x} + p\times \sum_{k=0}^n \lambda(k)\times\sum_{l = 0}^{k} \left( \begin{bmatrix} -\mb{CWBA} & \mb{c}_1 \end{bmatrix} \cdot \begin{bmatrix} \mb{x} \\ \bar{z} \end{bmatrix} \right)_{[l]}\label{eqn:rocii-form1}\\
%   &= \mb{1}^T \mb{B} \mb{A} \mb{x} + p\times \sum_{k=0}^n \xi_k \times \left( \begin{bmatrix} -\mb{CWBA} & \mb{c}_1 \end{bmatrix} \cdot \begin{bmatrix} \mb{x} \\ \bar{z} \end{bmatrix} \right)_{[k]},\label{eqn:rocii-form2}
% \end{align}
% where $\xi_k = \sum_{l = 0}^k \lambda(l) = \mathbb{P} [\vert \mathcal{S} \vert \le k]$ is the cumulative distribution function of the prior probability of $\lambda(k)$.
% Thus, $\xi_k \ge \xi_{k-1}$, and ROCII is still a convex optimization problem.
% A direct methods to solve ROCII is to use \refeq{eqn:rocii-form1} and the analysis of ROCPI. This will introduce $\mathcal{O}(n^2)$ slack variables, and is not practical for large-scale networks in reality.
% Note that main challenge is the non-continuity of objective in \refeq{eqn:rocii-form2}. Thus, we develop a projected sub-gradient method to solve this problem.
% The algorithm is shown in \refalg{alg:projected-sub-grad}.
% In \refalg{alg:projected-sub-grad}, we solve ROCII in \refeq{eqn:rocii} with objective in \refeq{eqn:rocii-form2} excluding the box constraint $\mb{0} \le \mb{x} \le \mb{s}$. Then, at the end of each iteration, we project the updated $\mb{x}$ onto the box area $\mb{0} \le \mb{x} \le \mb{s}$.
% The time complexity is $\mathcal{O}(n\log n \cdot iter)$, where $n\log n$ comes from the sort procedure in each iteration.
% Note that we do not introduce any slack variables or additional constraints, and thus, the projected sub-gradient method is scalable to large networks.
% It is worth to mention that since ROCPI is a special case of ROCII, it can also be solved with the projected sub-gradient method if the network size is sufficiently large.

% \begin{algorithm}[!t]
%   \SetAlgoLined
%   % \KwIn{Adjacency matrix $\mb{W}$, initial internal opinion $\mb{s}_0$, stubbornness $\mb{A}$, control budget $\mu$, perturbation coefficient $p$, prior distribution $\lambda(\hat{k})$, Number of iterates $m$, Initial step size $\beta_0$\;}
%   \KwIn{control budget $\mu$, prior distribution $\lambda(k)$, Number of iterates $m$, Initial step size $\beta_0$\;}
%   \KwOut{optimal controlled internal opinion $\mb{x}^*$}
%       Calculate parameters: 
%       $\mb{B} \leftarrow [\mb{I} - (\mb{I} - \mb{A})\mb{W}]^{-1}$,
%       $\mb{c}_0 = \mb{1}^T\mb{BA}$, $\mb{c}_1 \leftarrow (\mb{1}^T \mb{B}(\mb{I} - \mb{A}))^T$, $\mb{c}_2 \leftarrow \mb{WBAs}$, $\mb{C} \leftarrow \diag{\mb{c}_1}$, $\mb{M} \leftarrow [-\mb{C}\mb{WBA}, \mb{c}_1]$, $\xi(k) \leftarrow \sum_{l = k}^{n} \lambda(l)$
      
%       Build Inequality constraints:
%       $
%       \mb{A}_{ub} =
%       \left[\begin{array}{cc}
%       -\mb{1}^T & 0 \\
%       \mb{BA}   & -\mb{1}
%       \end{array}\right],
%       \mb{b}_{ub} = [\mu - \mb{1}^T\mb{s}_0,~ \mb{0}^T]
%       $
      
%       Initialize $\mb{x} = [\mb{s}^T, \max(\mb{s})]^T$\;
      
%       $\tilde{f}^* \leftarrow +\infty$, $\mb{x}^* \leftarrow \mb{s}$\;
      
%       \For{$iter \le m$}{
%           $\beta = \beta_0/ \sqrt{iter}$\;
%           \eIf{$\mb{A}_{ub}\cdot \mb{x} \preceq \mb{b}_{ub}$}{
%               Calculate $\mb{y} = \mb{Mx}$\;
              
%               Sort $y_i$ and so that $y_{[1]} \ge \cdots y_{[n]}$\;
              
%               Calculate current objective $f\leftarrow \mb{c}_0^T \mb{x} + p\cdot \sum_{l = 1}^{n} \xi(l) y_{[l]}$\;
              
%               \textbf{if} $f < f^*$ \textbf{then} $f^* \leftarrow f$, $x^* \leftarrow x$\;
              
%               $\mb{g} \leftarrow \mb{c}_0 + \sum_{l = 1}^{n} \xi(l) \cdot \mb{M}[i, :]^T$\;
%           }{
%               Find one index $i$ that $\mb{A}_{ub}[i, :] \mb{x} > \mb{b}_{ub}[i]$\;
              
%               $\mb{g} \leftarrow \mb{A}_{ub}[i, :]^T$\;
%           }
          
%           Update $\mb{x} \leftarrow \mb{x} - \beta \times \mb{g}$\;
          
%           \For{$i = 1, \cdots, n$}{
%               \textbf{if} $\mb{x}[i] < 0$ \textbf{then} $\mb{x}[i] \leftarrow 0$\;
%               \textbf{if} $\mb{x}[i] > \mb{s}[i]$ \textbf{then} $\mb{x}[i] \leftarrow \mb{s}[i]$\;
%           }
%       }
      
%       $\mb{x}^* \leftarrow \mb{x}[1:n]$
      
%       \caption{Projected subgradient algorithm for ROCII.}
%   \label{alg:projected-sub-grad}
% \end{algorithm}

